Image-to-GPS Verification Through A Bottom-Up Pattern Matching Network

The image-to-GPS verification problem asks whether a given image is taken at a claimed GPS location. In this paper, we treat it as an image verification problem -- whether a query image is taken at the same place as a reference image retrieved at the claimed GPS location. We make three major contributions: 1) we propose a novel custom bottom-up pattern matching (BUPM) deep neural network solution; 2) we demonstrate that the verification can be directly done by cross-checking a perspective-looking query image and a panorama reference image, and 3) we collect and clean a dataset of 30K pairs query and reference. Our experimental results show that the proposed BUPM solution outperforms the state-of-the-art solutions in terms of both verification and localization.

==> dataset.tex <==
\section{Dataset}\label{sec.dataset}
In order to train location verification network, we need paired query image and reference image 1) share same GPS coordinate and 2) are places more likely to be falsified on Internet. We followed below four steps to collect dataset
%\subsection{Location Filtering}
%Not all images interest us. e.g. landscape photo of mountains or sea are too common to verify and are very possible to be modified for not malicious purpose. While photos taken in urban area, especially places rally or protest are more likely to happen, are vulnerable to tampering. To collect photos of latter type. We referenced \cite{mccarthy2006places} to find these potentially modified places (PMP).
%We used {\it Google Places API} to request PMP's GPS information throughout the United States. A formatted request composed of place type, zip code and state, e.g. {\tt government+office,+New+York,+NY+10001}, is sent to {\it Google Places}. PMP images are going to be collected according to GPS coordinate in the returned result.

\subsection{Query Image Source}
{\it Mapillary}\footnote{www.mapillary.com}, a photo sharing website 1) supports GPS coordinate search 2) with high GPS accuracy and 3) user uploaded, is selected as first source of query images. We sent request with GPS coordinate as center and limited search range within 100 meters. Among returned results, the one nearest to requested coordinate is chosen as query image of the location. The disadvantage of {\it Mapillary} is that most of its photos are taken on the road, which results in too many meaningless photos containing only roads and no landmarks. \\
Another dataset containing 500 samples was collected from {\it Wikicommons} by manually verifying GPS location. These images advances ones from {\it Mapillary} in 1) higher confidence (have been verified by human) and 2) landmarks detectable, i.e. contain enough clues to verify. \\
Third dataset is from \cite{shibuyadata}, which contains 
In the experiment, 25,000 samples from {\it Mapillary} are used as training dataset. Three different testing datasets are 1) 5,000 samples from {\it Mapillary} 2) 500 samples from {\it Wikicommons} 3) 947 samples of {\it Shibuya}.\footnote{These numbers are of positive samples} Negative samples are generated by randomly pairing query image with reference image (which has different GPS location) from same dataset, in order to make sure they follow same distribution as positive samples. Number of negative samples is same as positive samples. 

\subsection{Reference Image Source}
{\it Google Street View}, which has 360\degree panorama images, is chosen as reference image source. Panorama image are retrieved using same GPS coordinate as query images and requests are constrained to outdoor source images. A third party program\footnote{https://github.com/Jam3/extract-streetview} is used to download panorama images.

\subsection{Data Cleaning}
Among retrieved query images, some does not contain any remarkable landmarks for location verification. In some photos collected form {\it Mapillary}, unremarkable things like cars, roads and sky are main component of image instead of building structures. To eliminate these weak clued samples which is difficult even for human to verify location, a {\it VGG}\cite{} network pretrained on {\tt Place365} dataset is used to clean data. Images of highest probability being {\tt highway, sky etc.}\footnote{All negative classes: \tt{clean room, forest road, highway, sky, volcano}} are removed from dataset. 
